Nonlinear differential equations on non-compact domains

We present some results in the analysis of non-compact differential equations on unbounded domains.

==> biblio.tex <==
@BOOK{Adams,
author={Adams},
title={Sobolev Spaces},
publisher={Academic Press},
year=1975
} 


==> intestaztesi.tex <==
\magnification=\magstep1
\hsize=13truecm
\vsize=24truecm
\hoffset=1.7truecm
\voffset=2truecm
\font\piccolo=cmr10 at 8pt
\font\doctor=cmsl10 at 11pt
\font\biasco=cmr10 at 11pt
\font\grande=cmbx10 at 20pt
\font\bft=cmbx10 at 11pt
\font\grassetto=cmbx10
\font\candidate=cmcsc10 at 11pt
\quad
\medskip
%\vskip1truecm

\centerline{\grande Nonlinear differential equations}
\vskip0.2truecm
\centerline{\grande on non-compact domains }


\vskip10truecm




\line{\candidate Candidate\hfill Supervisors}
\vskip.3truecm
\line{\biasco Simone Secchi\hfill Prof. Antonio Ambrosetti}
%\vskip.3truecm
%\line{\biasco\hfill Prof. Charles A. Stuart} 

\vskip4truecm


\centerline{\biasco Thesis submitted for the degree of {\doctor Doctor Philosophiae}}


\vskip0.3truecm

\centerline {\biasco Academic Year 2001-2002}

%\thispagestyle{empty}

%\pagebreak
\nopagenumbers
\end{document}


==> junk/partappe.tex <==
\part{Appendix}

